Targeting Makes Sample Efficiency in Auction Design

This paper introduces the targeted sampling model in optimal auction design. In this model, the seller may specify a quantile interval and sample from a buyer's prior restricted to the interval. This can be interpreted as allowing the seller to, for example, examine the top $40$ percents bids from previous buyers with the same characteristics. The targeting power is quantified with a parameter $\Delta \in [0, 1]$ which lower bounds how small the quantile intervals could be. When $\Delta = 1$, it degenerates to Cole and Roughgarden's model of i.i.d. samples; when it is the idealized case of $\Delta = 0$, it degenerates to the model studied by Chen et al. (2018). For instance, for $n$ buyers with bounded values in $[0, 1]$, $\tilde{O}(\epsilon^{-1})$ targeted samples suffice while it is known that at least $\tilde{\Omega}(n \epsilon^{-2})$ i.i.d. samples are needed. In other words, targeted sampling with sufficient targeting power allows us to remove the linear dependence in $n$, and to improve the quadratic dependence in $\epsilon^{-1}$ to linear. In this work, we introduce new technical ingredients and show that the number of targeted samples sufficient for learning an $\epsilon$-optimal auction is substantially smaller than the sample complexity of i.i.d. samples for the full spectrum of $\Delta \in [0, 1)$. Even with only mild targeting power, i.e., whenever $\Delta = o(1)$, our targeted sample complexity upper bounds are strictly smaller than the optimal sample complexity of i.i.d. samples.

==> 01bounded_single.tex <==
\subsection{$[0,1]$-Bounded Distributions}
We first consider the case that the data holder owns the true distribution.
Our algorithm is to divide the whole quantile space into small intervals of length $d$. 
For each quantile $q(q=kd,k\in\mathbb{N},k\le 1/d)$, we query for one sample from $[q-e, q+e](e\le d/2)$. Then we estimate the revenue of the quantile $q$ by the returned value, say, $\tilde v(q)$, times $q$. Among all the values returned, we select the value with the largest estimated revenue, namely $\tilde v_s$, as the reserved price. We suppose the corresponding quantile of $\tilde v_s$ w.r.t. true distribution is $\tilde q_s$ and $\tilde v_s$ is returned when we query around the quantile $q_s$. Suppose the optimal quantile and its corresponding value are $q^*$ and $v^*$. 
We first show that, the revenue of this algorithm $\tilde v_s \cdot \tilde q_s$ is close to optimal.
\begin{lemma}
$\tilde v_s \cdot \tilde q_s \ge q^*\cdot v^* - 2d -3e$. 
\end{lemma}
\begin{proof}
If $q^*<2d+3e$, the lemma holds trivially.
Otherwise we select the quantile which is the largest queried quantile among all the quantiles at least $d$ smaller than $q^*$ and we denote it as $q_b$ and we denote its corresponding quantile as $q_{b}$. When we query around the quantile $q_b$, suppose we get a returned value $\tilde v_b$ and the corresponding quantile of $\tilde v_b$.
We have the following inequalities:
\begin{gather*}
    q_b -e \le \tilde q_b \le q_b + e,\quad q_s-e\le \tilde q_s\le q_s+e\\
    \quad q^* -2d - e  <q_b < q^* -d +e, \\
    q_s \cdot \tilde v_s \ge q_b \cdot \tilde v_b,\\
    \tilde q_b < q^*,\quad \tilde v_b >v^*.\\
\end{gather*}
Therefore we have the inequality
\begin{align*}
    \tilde q_s\cdot \tilde v_s &\ge (q_s -e)\cdot \tilde v_s \\
    &\ge q_b\cdot \tilde v_b -e \cdot \tilde v_s\\
    &\ge (q^* -2d -e)\cdot v^* -e(\tilde v_b +\tilde v_s)\\
    &\ge q^*\cdot v^* -(2d+e)\cdot v^* - e\cdot \tilde v_b -e\cdot\tilde v_s\\
    &\ge q^*\cdot v^* -2d-3e.
\end{align*}
\end{proof}
Thus if we let $d=\epsilon/4$ and $e=\epsilon/8$, $\Theta(\epsilon^{-1})$ queries are enough to get a $1-\epsilon$ approximation of maximum auction revenue, under the condition that the data holder returns a value in the quantile interval with respect to the true distribution.\\\\
Then we consider the case that the data holder returns samples empirically. 
The statement is similar to the regular case.
\begin{lemma}
If the data holder has $m=\Omega(\epsilon^{-2}\cdot \log{(\delta^{-1}\epsilon^{-1})})=\tilde\Theta(\epsilon^{-2})$ samples and the seller queries for a quantile interval $[q-e/2, q+e/2](q>e)$, with $e=\Theta(\epsilon)$, the data holder first picks a quantile $q_r$ in the queried quantile interval randomly and return a value with this quantile empirically. Then the sample value falls in the quantile interval $[q-e,q+e]$ with probability at least $1-\epsilon\cdot \delta$.
\end{lemma}
\begin{proof}
    We consider the situation when a returned value falls out of the quantile interval. This would happen if the number of samples with smaller quantile, denoted as $m_l$ than $q-e$ is smaller than $q_r\cdot m$ or the number of samples with smaller quantile than $q+e$, denoted as $m_h$ is larger than $q_r\cdot m$.
    Therefore we use Chernoff bound similarly as the regular case and we have:
\begin{align*}
    Pr\{m_l<(q-e)m \text{ or } m_h\} &\le Pr\{m_l<(q-e)m\}+Pr\{m_h>(q+e)m\}\\
    &\le Pr\{m_l<\left(1-\frac{(e/2)m}{(q-e/2)m}\right)\cdot (q-e/2)m\} +\\
    &\quad Pr\{m_h>\left(1+\frac{(e/2)m}{(q+e/2)m}\right)\cdot (q+e/2)m\}\\
    &\le e^{-c{\left(\frac{e}{q}\right)}^2\cdot q\cdot m}\\
    &= e^{-c\frac{e^2}{q}m}.
\end{align*}
Since we have $q\le 1$ and $m=\Omega(\epsilon^{-2}\cdot \log{(\delta^{-1}\epsilon^{-1})})$, we get $1-e^{-c\frac{e^2}{q}m}\ge 1-e^{-c\cdot e^2\cdot \epsilon^{-2}\cdot \log{(\delta^{-1}\epsilon^{-1})}}\ge 1-\epsilon\cdot \delta$.
\end{proof}

\begin{theorem}
% In a single buyer $[0,1]$-bounded case. By any targeted sample algorithm based on query on quantiles, if the algorithm want to get an expected loss less than $\epsilon$, the number of samples required by the algorithm should be $\tilde \Omega(\epsilon ^{-1})$.
In the case of a single buyer with $[0,1]$-bounded distribution, any targeted sample algorithm based on quantile query must query $\tilde \Omega(\epsilon ^{-1})$ samples to obtain a revenue with an additive loss of at most $\epsilon$.
\end{theorem}
\begin{proof}
We use Yao's Minimax Principle (Lemma~\ref{lem:Yao}) to prove this theorem. First we claim that, without loss of generality, we can assume that when the algorithm query for a value from the data holder, it queries at a precise quantile point $q$. Because if an algorithm query for a random value in a quantile interval $(q_l,q_h)$, this step can be replaced by 2 steps: (1) uniformly pick a quantile $q$ in the interval $(q_l,q_h)$; (2) query for the value at this quantile $q$. This simplification provides convenience for the following proof.
    
    By Lemma~\ref{lem:Yao}, we only need to prove that any deterministic algorithm cannot give a reserve price with $(1-\epsilon)$ revenue with probability more than $(1-\delta)$ on a fixed distribution of the bidder's value distributions. So we construct it as follows:
    
    % A bidder's value distribution is denoted as $D_s$ where $s$ is an integer in $[0,\frac1\epsilon)$. The revenue-quantile curve under $D_s$ is defined as:
    % $$R^{D_s}(q)=\left\{
    % \begin{aligned}
    % &q,\quad &(0\le q< \frac12)\\
    % &\frac1{1+2\epsilon}\cdot (q-\frac12-s\epsilon),\quad&(\frac12+s\epsilon\le q<\frac12+(s+1)\epsilon)\\
    % &\frac12,\quad &(\text{else where})\\
    % \end{aligned}\right.
    % $$

% \syh{I gave a new fixed distribution here, and the figure is drawn according to this distribution}
    A bidder's value distribution is denoted as $D_s$ where $s$ is an integer in $[0,\frac{1}{2\epsilon})$. The revenue-quantile curve under $D_s$ is defined as:
    $$R^{D_s}(q)=\left\{
    \begin{aligned}
    &q,\quad &(0\le q< \frac12)\\
    &\frac1{2}\cdot (q+\frac12-s\epsilon),\quad&(\frac12+s\epsilon\le q<\frac12+(s+1)\epsilon)\\
    &\frac12,\quad &(\text{else where})\\
    \end{aligned}\right.
    $$
    
Fig.~\ref{fig:01boudned} shows the $R-q$ curve of $D_s$. 
    \begin{figure}
    
        \centering
        \includegraphics[scale=0.6]{il_4.png}
        \caption{The $R-q$ curve of one $D_s$ we constructed for some $s$. The hill is in interval $[\frac12+s\epsilon,\frac12+(s+1)\epsilon) $. Note that the slope of the small hill is always 1/2, so the $R-q$ curve is well defined. }
        \label{fig:01boudned}
    \end{figure}
    We let $s$ follows a uniform distribution in the set of integers in $[0,\frac{1}{2\ep})$. 
    This forms a distribution of the bidder's value distribution based on definition of $D_s$. 
    Now we analyse how many samples are necessary for a deterministic algorithm to approximate the optimal result with an additive error of at most $\ep$.
    
    First let us see how this distribution's $R-q$ curve looks like. In the quantile interval $[\frac12,1]$ the $R-q$ curve is almost horizontal at an altitude $\frac12$, except some small `hills' in small sub-intervals, each with a height of at least $\frac{1+\epsilon}2$ (as illustrated in Fig.~\ref{fig:01boudned}). 
    The hill might occur at $\frac1\epsilon$ different places. If an algorithm fail to report a value at the hill, then the approximation fails. 
    Now suppose the algorithm takes $k$ samples, then it can see whether there exists a hill at at most $k$ places. 
    Obviously the optimal algorithm based on these $k$ samples must have the following form: (1) query at $k$ places where the hill might be. (2) return the corresponding value if it see the hill, or return another value at other places that has not been queried. 
    The probability of failing is at least:
    $$p_f=\frac{\frac1\epsilon-k}{\frac1\epsilon}\cdot\left(1-\frac1{\frac1\epsilon-k}\right)=1-\epsilon(k+1).$$
    We hope $p_f\le\delta$, so we must have $k>\frac{1-\delta}\epsilon-1=\Omega(\epsilon^{-1})$.
\end{proof}


==> MHR_single.tex <==

\subsection{MHR}
The algorithm we use in the MHR case is totally the same as that of the regular case, except the truncation step. In the regular case, we truncate both of the two sides of the whole quantile interval for $\Theta(\epsilon)$ length. In the MHR case, we truncate $1/e$ for each side. That is to say, the initial interval should be $[a_0,b_0]=[1/e, 1-1/e]$. Note that in the MHR case, we could guarantee that there should be a quantile with maximum revenue in the interval $[1/e, 1-1/e]$. The convexity of the revenue curve still holds. Thus $O(\log\epsilon^{-1})$ samples are enough to find a $1-\epsilon$ approximation of the maximum revenue. Since for any quantile $q$ we query in the algorithm, we have $q=\Theta(1)$. Each time we query, we get a $e^{-c\cdot \epsilon^2\cdot q\cdot m}$ probability to fail. In order to get a final success rate $1-\delta$, we only need to let the number of data holder's samples be $m=\tilde\Theta(\epsilon^{-2}\cdot\log{\delta^{-1}})$. 

\xiangning{Will update ref table.}
Recall that in Table~\ref{table:single1}, for regular or $[0,1]$-bounded distributions, the size of data set for the corresponding upper bound almost matches the sample complexity lower bound in \cite{HuangMR/2018/SICOMP}, up to logarithmic factors. 
For MHR distributions, since the sample complexity of the lower bound for MHR distributions is $\Omega(\epsilon^{-1.5})$(\cite{HuangMR/2018/SICOMP}), there is still space for improvement.
This is mainly because the definition of MHR distributions indeed indicates a stronger concavity of its revenue-quantile curve, than that of regular distributions. 
The state-of-the-art standard sample complexity upper bound \cite{HuangMR/2018/SICOMP}, improved the former upper bound\cite{DRY15} from $\tilde{O}(\epsilon^{-2})$ to $\tilde{O}(\epsilon^{-3/2})$ by a subtle proof based on the stronger concavity. 
There may be ways to make full use of this strong concavity in our model.
A better upper bound of number of queries, and a non-trivial lower bound(more concrete than $\tilde{\Omega}(1)$) are still open problems.




==> general_multi.tex <==
% ================ OLD MATERIALS
We construct an algorithm for which we could take at most $m$ samples for each type of distribution.

We will show that, there always exists a threshold of virtual value such that: (1)Ignoring values with virtual value that below this threshold will lose only $\epsilon$-fraction of the optimal, and (2)a much smaller numbers of samples is enough to learn the nearly optimal mechanism. 
First we show the existence of such a threshold.
The proof is mainly based on a division of virtual value space.
\begin{lemma}\label{lem1}
    For regular or MHR product value distribution $\bm{D}$, we denote the virtual value function of the distribution $D_i$ as $w_i$, there exists a set of quantiles $\bm{\theta}=(\theta_1,\theta_2,\cdots,\theta_n)\in [0,1]^n$, such that:
    \begin{itemize} 
    \item[1.] There exists a virtual value $w^*$, s.t. $\forall i, q_i\in[0,1]$ if $q_i\ge \theta_i$,  $w_i(q_i)\le w^*$; if $q_i\le \theta_i$, $w_i(q_i)\ge w^*$.
    \item[2.] $\Pi_i(1-\theta_i) \le \epsilon$.
    \item[3.] $\sum_{1\le i\le n}\theta_i \le \tilde \Theta(1)$.
    \end{itemize}
\end{lemma}

\begin{proof}
For any virtual value $w$, for each $i$ we define:
$$\bar \theta_i(w):=\sup\{q:w_i(q)\ge w\}~.$$
$$\underline \theta_i(w):=\inf\{q:w_i(q)\le w\}~.$$
Since $\bm{D}$ is regular, every $\bar \theta_i$ and $\underline \theta_i$ are decreasing in $w$. 
Further define $\bar f(w):=\Pi_i(1-\bar\theta_i(w))$ and similarly $\underline f$, and they are increasing in $w$.
By definition, we have $\bar f(w) \le \underline f(w)$ and $\underline \theta_i(w)\le \bar \theta_i(w)$, $\forall w,i$. 
For any $w_1\le w_2$, for each $i$, $\underline \theta_i(w_1)\ge \bar \theta_i(w_2)$. 
This implies $\underline f(w_1)\le \bar f(w_2)$.
We can verify that 
$$\lim_{w\rightarrow w_1+} \bar f(w) =\underline f(w_1) ~.$$ 
$$\lim_{w\rightarrow w_2-} \underline f(w) =\bar f(w_2) ~.$$ 

% Note that $\lim_{w\rightarrow +\infty}\bar f(w)=1$, there must exist an upper bound $W$ of all possible virtual values such that $\bar f(W)>\epsilon$. 
% Now continually decrease $w$ from $W$ to find a $\bm{\theta}$ that simultaneously satisfies condition 2 and 3.
By $\lim_{w\rightarrow -\infty}\bar f(w)=0$, we can define $w':=\inf \{w:\bar f(w)\ge \epsilon\}$ and $w'\neq -\infty$.
We then show the existence case by case.
\begin{itemize}
    \item If $\bar f(w')=\epsilon$, then let $w^*=w'$ and $\bm{\theta}=\bm{\bar \theta}(w')$. Then 1 and 2 are directly satisfied. For 3,
    \[
        \sum_{1\le i\le n} \theta_i =n-\sum_{1\le i\le n}(1-\theta_i)\le n(1-{\epsilon}^{\frac1n})\le\ln\epsilon^{-1} 
        ~.
    \]
    \item If $\bar f(w')> \epsilon$, then $\forall w<w'$, $\bar f(w)<\epsilon$ by the definition of $w'$.
        We can always find a $w<w'$ s.t. $\underline f(w)> \epsilon$.
        Suppose this is not true, then $\forall w<w'$, $\underline f(w)\le \epsilon$. 
        This implies $\bar f(w')=\lim_{w\rightarrow w'-} \underline f(w)\le \epsilon$, which is a contradiction. 
        Now we can set this $w$ to be $w^*$. 
        Also note that $\Pi_i(1-\bar\theta_i)$ is continuous in $\bm{\theta}$, and thus, there must exists $\bm{\underline \theta}(w)\preceq \bm{\theta}\preceq \bm{\bar \theta}(w)$ s.t. $\Pi_i(1-\theta_i)=\epsilon$. 
        This implies condition 3 as discussed in the first case.
    \item If $\bar f(w') < \epsilon$, then we must have $\underline f(w')\ge \epsilon$. 
        In fact, if $\underline f(w')<\epsilon$, then $\lim_{w\rightarrow w'+} \bar f(w) =\underline f(w')<\epsilon$, which contradicts the definition of $w'$. Then it's the same as the second case, we set $w^*=w'$ and there exists $\bm{\underline \theta}(w')\preceq \bm{\theta}\preceq \bm{\bar \theta}(w')$ satisfy the conditions.
\end{itemize}
\end{proof}
\begin{lemma}\label{lem11}
    For $[0,1]$-bounded product value distribution $\bm{D}$, we denote the ironed virtual value function of the distribution $D_i$ as $w_i$, there exists a set of quantiles $\bm{\theta}=(\theta_1,\theta_2,\cdots,\theta_n)\in [0,1]^n$, such that:
    \begin{itemize} 
    \item[1.] There exists a virtual value $w^*$, s.t. $\forall i, q_i\in[0,1]$ if $q_i\ge \theta_i$,  $w_i(q_i)\le w^*$; if $q_i\le \theta_i$, $w_i(q_i)\ge w^*$.
    \item[2.] $\Pi_i(1-\theta_i) \le \epsilon$.
    \item[3.] $\sum_{1\le i\le n}\theta_i \le \tilde \Theta(1)$.
    \end{itemize}
\end{lemma}
\begin{proof}
The proof is almost identical as Lemma \ref{lem1}. 
The only difference is that when we prove the existence of a $\bm{\underline \theta}(w^*)\preceq \bm{\theta}\preceq \bm{\bar \theta}(w^*)$ s.t. $\Pi_i(1-\theta_i)=\epsilon$, we cannot directly choose this $\bm{\theta}$.
This is because each $\theta_i$ cannot be inside any ironed interval. 
Otherwise, consider the distribution by setting all the values with quantile greater than $\theta_i$ to $0$. 
The new distribution in general will have a very different way of ironing for the part with quantile less than $\theta_i$, and thus will lead to a big loss in revenue. 

The solution is simple. 
Starting from $\bm{\underline \theta}(w^*)$, in the $i$-th round we change its $i$-th coordinate to $\bar \theta_i(w^*)$, and stop until condition 2 is satisfied. 
Then $\sum_{1\le i\le n}\theta_i$ will increase at most $1$ each time we change.
Note that for a $\bm{\theta}$ if condition 2 is not true, then condition 3 must hold:
 $$\sum_{1\le i\le n} \theta_i =n-\sum_{1\le i\le n}(1-\theta_i)\le n(1-{\epsilon}^{\frac1n})\le\ln\epsilon^{-1} ~,$$
So we have $\sum_{1\le i\le n}\theta_i\le \tilde \Theta(1)$ before the last change.
and when we stop the process, we still have $\sum_{1\le i\le n}\theta_i\le \tilde \Theta(1)$.
\end{proof}
\begin{comment}
\begin{proof}
The proof of this lemma is simple. First consider the case that the virtual value functions $w_i(q)$ are strictly monotone for all bidders. Then for any virtual value $\phi$, there exists a unique quantile $q_i$ for each bidder $i$ such that $w(q_i)=\phi$,so that there exists the inverse function $q_i=w_i^{-1}(\phi)$. A special case is that $\phi$ may not be a possible virtual value for a bidder, so we generalize this function as follows: let $w^{-1}(\phi)=0$ iff $w_i(0)\le\phi$ and $w^{-1}(\phi)=1$ iff $w_i(1)\ge\phi$. Now $w_i^{-1}(\phi)$ are well defined as continuous functions on $\phi$.
\xiangning
{
It seems a wrong $w^{-1}(\cdot)$, because it may make $p(\phi)$ jump to 0 or 1 when such $\phi$ is off from the boundary. 
Unless the distribution is assumed to be differential.
You may try a standard way to handle discontinuous, by defining 2 functions with inf and sup to locate all the possible positions of $\theta_i$.
}
Consider a new function which is still continuous: $$p(\phi)=\prod_{1\le i\le n} (1-w_i^{-1}(\phi)).$$
We have that $p(+\infty)=0$ and $p(-\infty)=1$, so there exist $\phi=w^*$ such that $p(w^*)=\epsilon$. Let $\theta_i=w_i^{-1}(\phi)$ then the 1st and 2nd claim are satisfied. The 3rd claim is directly deduced from the 2nd one:
$$\sum_{1\le i\le n} \theta_i =n-\sum_{1\le i\le n}(1-\theta_i)\le n(1-{\epsilon}^{\frac1n})\le\ln\epsilon^{-1}$$
Up to now we have proved the lemma in the case with strict monotonicity, in the general case, this monotonicity is weak. So that $w_i^{-1}(\phi)$ might not be well defined, as a $\phi$ might be mapped to any $p$ in some interval. But this does not influence the `continuity' of this function, and we can arbitrarily choose $\theta$ in this interval. So the proof of this lemma is done.
\end{proof}

\hyh{I write an alternative proof of different style here, please see if it is appropriate.}
\\

The intuition of the proof here is as follows: first find out an upper bound $\bar \phi$ of the ironed virtual values of all bidders. Initially let $\phi=\bar\phi$ and we continuously decrease its value until the conditions we require in the lemma are satisfied. 

\begin{proof}
First we claim that for any $\phi$, there exists a non empty set of quantiles $S_i(\phi)$ such that $\forall i$, $\forall \theta_i\in S_i(\phi)$  
\begin{itemize}
    \item $w_i(\theta_i)=\hat w_i(\theta_i)$, where $\hat w_i(q)$ is the function of ironed virtual value on $q$).
    \item $\hat w_i(q)\ge \phi$ if $q<\theta_i$; $\hat w_i(q)\le \phi$ if $q>\theta_i$.
\end{itemize}
This is easy to prove as that the ironed revenue-quantile curve is concave. So a bidder's virtual value-quantile function is non-increasing. If it keep constant in some quantile interval, the 2 end points of this interval must satisfy $\phi =w_i(\theta_i)=\hat w_i(\theta_i)$ (this 2 quantiles are exactly the 2 elements of $S_i(\phi)$). In other cases the correctness of this claim is trivial.

Now we let $\phi$ be $\bar\phi$ which is larget enough such that $w_i(0)\le\bar \phi$, $\forall i$. This also means that $\theta_i\in S_i(\bar\phi)=\{0\}$, $\forall i$. Then we can continuously decrease $\phi$, and renew values of $\theta_i$ to be element of the current $S_i(\phi)$. Whenever some $S_i(\phi)$ have multiple elements, we stop decreasing $\phi$, choose a bidder $i$ and start changing $\theta_i$ to be different elements of $S_i(\phi)$. If no such process can be done we continue to decrease $\phi$. The whole process stops until $\prod_i(1-\theta_i)\le \epsilon$. Now there might be 2 cases:

\begin{itemize}
    \item if exactly $\prod_i(1-\theta_i)= \epsilon$. Then these $\theta$ directly satisfies the lemma because 
    $$\sum_{1\le i\le n} \theta_i =n-\sum_{1\le i\le n}(1-\theta_i)\le n(1-{\epsilon}^{\frac1n})\le\ln\epsilon^{-1}.$$
    \item if $\prod_i(1-\theta_i)< \epsilon$, then it must be the following case: the quantile of some $j$-th bidder is increased in the last step from $\theta_j^l$ to $\theta_j$. (i.e. for the current virtual value $\phi$, $\{\theta_j^l,\theta_j\}\in S_i(\phi)$) So we deduce that: $\prod_{i\ne j}(1-\theta_i)\cdot \theta_i^l> \epsilon$. Thus we have:
    $$\sum_{1\le i\le n} \theta_i =n-\sum_{1\le i\le n}(1-\theta_i)\le n(1-{\epsilon}^{\frac1n})-\theta_i^l+\theta_i\le\ln\epsilon^{-1}+1.$$
\end{itemize}

So when the process stops the virtual value $w^*=\phi$ with the current quantiles of bidders satisfies the claims in the lemma.
\end{proof}
\end{comment}

\begin{lemma} \label{lem2}
 Given a quantile vector $\bm{\theta}$ in lemma \ref{lem1}. There exists a quantile vector $\bm{\theta'} = \{\theta'_1,\theta'_2,\cdots,\theta'_n\}$ and a small const $\epsilon_b$ such that:
\begin{itemize}
\item[1.] $\forall i$, either $\exists k_i\in \mathbb{N}$ s.t. $\theta'_i=\epsilon_b \cdot 2^{k_i}$, or $\theta'_i= 1$.
\item[2.] $\Pi_i(1-\theta_i') \le \epsilon$.
\item[3.] $\sum_i \theta_i' = \tilde O(1)$
\end{itemize}
\end{lemma}

\begin{proof}
Round each $\theta_i$ to the smallest 2-power multiple of $\epsilon_b$ and select the minimum between this multiple and 1 would give such a satisfied $\bm{\theta'}$. Since each $\theta_i'$ is at most twice as much as the original $\theta_i$, the sum of the $\theta_i'$ is at most twice as much as the sum of $\theta_i$, that is also $\tilde O(1)$
\end{proof}
For any distribution $D$, we call any quantile vector with the properties in the lemma \ref{lem2} a \textbf{corresponding proper} quantile. \\

We define a truncation function on a distribution $t^{\min}_{q_i}$ such that for any distribution $D_i$ we truncate all the values with quantile more than $q_i$ to zero. That is to say $$q^{t^{\min}_{q_i}(D_i)}(v)\triangleq \left\{ 
\begin{array}{ll}
\min\{q^{D_i}(v), q_i\}& \text{if } v>0\\
1 & \text{if } v=0
\end{array}
\right..$$\\
Further, for any product value distribution $\bm{D}$ and any quantile vector $\bm{q}$ with the same dimension as $\bm{D}$, we define:
$$t_{\bm{q}}^{\min}(\bm{D}) \triangleq t_{q_1}^{\min}(D_1)\times t_{q_2}^{\min}(D_2) \times\cdots \times t_{q_n}^{\min}(D_n)$$.

\begin{lemma}
For each distribution $\bm{D}$, suppose there exists a quantile vector $\bm{\theta'}$ satisfying the conditions in lemma \ref{lem2}, then we have 
$$\opt {t_{\bm{\theta'}}^{\min}(\bm{D})}\ge (1-\epsilon)\opt{\bm{D}}$$ 
\end{lemma}
\begin{proof}
This is to simply divide the whole value space into two parts according to the vector $\bm{\theta}$ and the virtual value on the right part is always smaller than the left part. Since when there is at least one value fall in the left part, the Myerson on the truncated distribution would give the item to the buyer with the maximal virtual value, this would not bring revenue loss.
\end{proof}


\begin{comment}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\syh{Here we give out the definition of the piece-wise empirical distribution on the whole quantile interval [0,1].}
We announce our first mechanism: for buyer $i$ we take $m_d$ samples from the quantile interval $[0,\epsilon_b]$, take $m_d$ samples from the second quantile interval $[\epsilon_b, 2\epsilon_b]$, take $m_d$ samples from the third quantile interval $[2\epsilon_b,4\epsilon_b]$, $\cdots$. For buyer $i$, we take the samples until the interval $[\theta'_i/2,\theta'_i]$. Therefore we have taken at most $\log(1/\epsilon_b)\cdot m_d$ samples for each buyer. 

Define the following function: 
$$s_{m,n,\delta}(q)\triangleq \max\left\{0,q-\sqrt{\frac{2q(1-q)\ln(2mn\delta^{-1})}{m}}-\frac{4\ ln(2mn\delta^{-1})}{m} \right\}.$$ 

For a distribution $\bm{D}$, we abuse the notation by letting $s_{m,n,q}(D)$ denote a distribution such that for any value $v>0$ with quantile $q$ in $D$, its quantile in $s_{m,n,\delta}(D)$ is $s_{m,n,\delta}(q)$. Let $s_{m,n,q}(\bm{D})$ denote the product distribution obtained by applying $s_{m,n,q}$ to each coordinate  of $\bm{D}$.

 Then we construct an empirical distribution $E_i$ based on this samples taken from buyer $i$:
For each quantile interval $[t_l, t_r]$ within which we asked for $m_d$ samples, each sample value has a equal probability of $\frac{t_r-t_l}{m_d}$ to be selected in the empirical distribution. Let $\tilde{E_i} = s_{m_d/\theta_i',n,\delta}(E_i)$. We define the product dominated piece-wise empirical distribution as 
$$\bm{\tilde{E}}=\tilde{E_1}\times \tilde{E_2}\times\cdots \tilde{E_n}.$$
\begin{theorem}
If we run the Myerson's optimal auction on the distribution $\bm{\tilde{E}}$ with $m_d=\tilde{O}(\epsilon^{-2})$, the revenue of this mechanism would bring a $1-\epsilon$ approximation of the optimal revenue. 
\end{theorem}

\begin{proof}
The proof is broke down into the several lemmas as the following.
\begin{lemma}
With probability at least $1-\delta$, we have $\bm{D}\succeq \bm{\tilde{E}}$.
\end{lemma}
\begin{proof}
Since the sampling density is always larger than $m_d/\theta_i'$ samples per unit quantile, there is less chance for each quantile to deviate from the original distribution. 
\end{proof}
Our proof sketch is to use revenue monotonicity as the follows:
\begin{align*}
\rev{M_{\bm{\tilde{E}}},\bm{D}} &\ge\opt{\bm{\tilde{E}}}\\
&\ge \opt{\tr{\bm{\tilde {E}}}}\\
&\ge (1-\epsilon)\cdot \opt{\tr{\bm{D}}}\\
&\ge (1-2\epsilon)\cdot \opt{\bm{D}}.
\end{align*}
We define a new function:
$$d_{m,n,\delta}\triangleq \max\left\{0,q-\sqrt{\frac{8q(1-q)\ln(2mn\delta^{-1})}{m}}-\frac{7\ ln(2mn\delta^{-1})}{m} \right\}.$$ 
Similarly as $s_{m,n,\delta}$, we extend this notation to the product distribution. For any product value distribution $\bm{D}$, and a quantile vector $\bm{\theta'}$, we define $d_{m_d,n,\delta,\bm{\theta_i'}}= d_{m/\theta_1',n,\delta}(D_1)\times d_{m/\theta_2',n,\delta}(D_2) \times \cdots \times d_{m/\theta_n',n,\delta}(D_n)$. We denote $d_{m,n,\delta,\bm{\theta_i'}}(\bm{D})$ as $\bm{\tilde{D}}$.

\begin{lemma}\label{lem5}
For any distribution $\bm{D}$ and a corresponding proper quantile vector $\bm{\theta'}$, with probability at least $1-\delta$, we have:
$$\tr{\bm{\tilde{E}}} \succeq d_{m_d,n,\delta,\bm{\theta'}}(\tr{\bm{D}}).$$
\end{lemma}
\begin{proof}
Similar as the original proof. 
\end{proof}
\syh{I think here the shaded quantile amount could be simpler, but for convenience, I use the original shading amount. After I have written them all, I would consider whether to use other cleaner quantiles.}
\begin{lemma} \label{lem3}
Suppose there is a distribution $D$ with bounded support in $[l,u]$ and there is point mass $p_l$ at the quantile point $l$ and a point mass $p_u$ at the quantile point $u$. If both point masses are at least $\frac{64\ln(2mn\delta^{-1})}{m}=\tilde \Omega(m^{-1})$, then we have: $$\dskl{D,d_{m,n,\delta} (D)} =\tilde O(\dfrac{1}{m} \ln(p_l^{-1}\cdot p_u^{-1}))$$  
\end{lemma}
\begin{proof}
This proof is shown in the STOC 2019 paper, lemma 10.
\end{proof}
\begin{lemma}\label{lem4}
For any product value distribtuion $\bm{D}$ and a corresponding proper quantile vector $\bm{\theta'}$, we let $\bm{D^T}= \tr{\bm{D}}$. Suppose that there exist $\bm{\bar v}$, $\beta \ge \opt{\bm{D}}$, $\bm{\theta '}$ and $p>0$ such that:
\begin{itemize}
    \item[1.] $\beta\ge p\bar v_i$ for all $i\in [n]$.
    \item[2.] $q^{D^T_i}(\bar v_i)$ is at least $p \epsilon^2 \cdot \theta_i'$ for all $i\in [n]$. \syh{I think here the quantile should be fixed to $p\epsilon^2 \cdot \theta_i'$}
    \item[3.] $\opt{t^{\max}_{\bar{\bm{v}}}(\bm{D^T})}\ge \opt{\bm{D^T}}-O(\epsilon \beta)$.
\end{itemize}
Then, there exists distributions $\bm{D'}$ and $\bm{\tilde{D'}}=d_{m_d,n,\delta,\bm{\theta_i'}}(\bm{D'})$ such that for any $m_d\ge \tilde{O}(p^{-1}\epsilon^{-2})$: 
\begin{itemize}
    \item [a)] $\bm{D'}$ and $\bm{\tilde{D}'}$ have bounded supports in $[0,p^{-1}\beta]$ coordinate-wise.
    \item [b)] $\opt{\bm{D'}}\ge \opt{\bm{D^T}}- 2\epsilon \beta$.
    \item [c)] $\bm{\tilde{D^T}} \succeq \bm{\tilde{D'}}$.
    \item [d)] $\dskl{\bm{D'}, \bm{\tilde{D'}}} = O(p\epsilon^2)$.
\end{itemize}
\end{lemma}
\begin{proof}
We let $\bm{\epsilon}$ be an $n$-dimension vector $(\epsilon, \epsilon,\cdots,\epsilon)$.
We simply let $\bm{D'} = t^{\min}_{\bm{\epsilon}} \circ t^{\max}_{\bm{\bar v}}(\bm{D^T})$.
%\newcommmand{\tmax}{\opt{t^{\max}_{\bm{\bar{v}}}(\bm{D^T})}} %% This is the optimal value of truncating the largest values properly.
\begin{itemize}
    \item [Part a)]
    The first condition implies that $\bar v_i\ge p^{-1} \beta$.
    \item [Part b)]
    By the third condition and revenue monotonicity, we have $$\opt{{\bm{D^T}}} \ge\opt{t^{\max}_{\bm{\bar{v}}}(\bm{D^T})} \ge \opt{{\bm{D^T}}} -O(\epsilon\beta).$$
    Therefore we have:
    \begin{align*}
        \opt{\bm{D'}}&=  \opt{t^{\min}_{\bm{\epsilon}} \circ t^{\max}_{\bm{\bar v}}(\bm{D^T})}\\
        &\ge (1-\epsilon) \opt{t^{\max}_{\bm{\bar{v}}}(\bm{D^T})}\\
        &\ge (1-\epsilon)(\opt{\bm{D^T}}-\epsilon\beta) \\
        &\ge \opt{\bm{D^T}} -O(\epsilon\beta).
    \end{align*}
    \item[Part(c)] Since $\bm{D'}$ is obtained by truncating bopth the top and the bottom ends of the distribution $D^T$. And the function $d_{m,n,\delta,\bm{\theta'}}$ is monotone function over distribution. 
    \item[Part(d)] For every bidder, since we have truncate the last $\epsilon$ part of the distribution and the first $p\epsilon^2\cdot \theta_i'$ amount of quantile, using the lemma \ref{lem3}, we have $p_u \ge  p\epsilon^2 \cdot \theta_i' =\tilde \Omega((m_d/ \theta_i')^{-1})$ and $p_l\ge \epsilon =\tilde \Omega((m_d/ \theta_i')^{-1}).$ Therefore by lemma \ref{lem3}, we have $\dskl{D'_i,\tilde {D'_i}}= \tilde O({\theta_i'/m_d})= \tilde{O}(p\epsilon^2 \cdot \theta_i')$. Since we have $\sum_i{\theta_i'}=\tilde{O}(1)$, we have:
    $$\dskl{\bm{D'},\bm{\tilde{D'}}} = \sum_i \dskl{D'_i,\tilde {D'_i}} = \tilde O(p{\epsilon^2}).$$
\end{itemize}
\syh{Since the original proof of part a), b), c) all works for the [0, 1]-bounded case, even after the truncation after $\bm{\theta'}$ (the [0,1]-bounded property still does not change after the truncation. We only need to prove the d) part. }
\end{proof}
\begin{corollary}\label{cor1}
Suppose that there is a product value distribution $\bm{D}$ with a corresponding quantile vector $\bm{\theta'}$, a satisfied $\bm{\bar v}$ and $p$ with $\beta = 1$, then with probability at least $1-\delta$, we have $\rev{M_{\bm{\tilde{E}}}, \bm{D}}\ge \opt{\bm{D}} -5\epsilon.$
\end{corollary}

\begin{proof}
With probability at least $1-2\delta$, we have $\bm{D}\succeq \bm{\tilde{E}}$. Therefore we have 
\begin{align*}
\rev{M_{\bm{\tilde{E}}},\bm{D}} &\ge\opt{\bm{\tilde{E}}}\\
&\ge \opt{\tr{\bm{\tilde {E}}}}\\
&\ge \opt{\bm{\tilde{D^T}}}\\
&\ge \opt{\bm{\tilde{D'}}}.\\
\end{align*}
Since $O(p^{-1}\epsilon^{-2})$ samples are sufficient to estimate the expected revenue of the two mechanism $\bm{D'}$ and $\bm{\tilde{D'}}$ up to an additive error $\beta \epsilon$, by part d) of lemma \ref{lem4} we have:
\begin{align*}
\opt{\bm{\tilde{D'}}} &\ge \opt{\bm{D'}} - 2\beta\epsilon\\
&\ge \opt{\tr{\bm{D}}} -2\epsilon\beta -2 \beta\epsilon\\
&\ge (1-\epsilon)\opt{\bm{D}} -4\beta\epsilon\\
&\ge \opt{\bm{D}} -5\epsilon.
\end{align*}
\end{proof} 
The rest thing is to find the $p$ and vector $\bm{\bar{v}}$ which could satisfy the three conditions in lemma \ref{lem3}. To find these, we simply let $p=1$, $\beta=1$ and
$\bar v_i = \sup\{v: q^{D_i} \ge \epsilon^2 \cdot \theta_i'\}.$

The first two conditions are satisfied naturally by the definition of $\bar v_i$ and the property of $[0,1]$-bounded distributions. We only need to prove the third condition.
\begin{align*}
    \opt{\bm{D^T}} - \opt{t^{\max}_{\bar{\bm{v}}}(\bm{D^T})}&\le \sum_i \textbf{Pr}\{\exists i \in [n]:v_i>\bar v_i\} \\
    &\le \sum_i \textbf{Pr}\{ v_i> \bar v_i\}\\
    &\le \sum_i \theta_i' \cdot \epsilon ^2\\
    &\le O(\epsilon^2)\\
    & =O(\epsilon).
\end{align*}
Therefore, by corollary \ref{cor1}, we could prove that with only $\tilde{O}(\epsilon^{-2})$ samples per buyer, we could get an additive error at most $\epsilon$ with probability at least $1-\delta$.
\end{proof} 
Since the $\bm{\tilde{E}}$ depends on the selection of the $\bm{\theta'}$,if we want to construct the $\bm{\tilde{E}}$ above, we need to enumerate all the types of $\bm{\theta'}$. This may be exponential in computational complexity. Therefore, we should give a more elaborated shading method. 
The method is to shade respectively for each quantile interval with $m_d$ samples. \\
We define a new distribution $\hat{E}_i$ based on the empirical distribution $E_i$. For each value $v$ in the respective empirical distribution $\bm{E}$, suppose $q^{E_i}(v)$ falls in the quantile interval $[t_l, t_r]$, in which we take $m_d$ samples from in the sampling method, we let  
$$
q^{\hat{E}_i}(v)= s_{m_d/(t_r-t_l),n,\delta}(q^{E_i}(v)).
$$
We let $$\bm{\hat{E}} = \hat{E_1} \times \hat {E_2} \times\cdots \times\hat{E_n}.
$$
We now consider the case in which the company returns the value accurately according to the quantile we query. The query method is as the following: in the original method, suppose we ask for $m_d$ values in each quantile interval $[t_l, t_r]$; In this case, the quantiles we are querying is isometrically distributed among this quantile, i.e., suppose $t_r-t_l = d$ we query the quantiles $t_l, t_l +d/m_d,t_l+2d/m_d,\cdots, t_r$. Then we suppose the empirical distribution is $E$, we apply $M_{\hat{E}}$ on the distribution $D$. 
\begin{lemma}
With probability at least $1-\delta$, we have $\bm{D} \succeq\bm{\hat{E}}$ if the data company has data at least $m_d / \epsilon_b$. 
\end{lemma}
\begin{proof}
Suppose that the data company has at least $m_d / \epsilon_b$ samples, then with probability at least $1-\delta$ and the data company answer our query accurately according to their dataset. By the Bernstein inequality, if the data company has data at least $m_d/\epsilon_b$, we denote the empirical distribution on the samples of the data company  as $\bm{E'}$. We have the following inequality holds for all the quantiles which are multuples of $\epsilon_b/m_d$ with probability at least $1-\delta$:
$$
\left\vert q^{E'_i}(v) -q^{D_i}(v)\right\vert \le \sqrt{\frac{2q(1-q)\ln(2m_d\cdot n\cdot \delta^{-1}\cdot \epsilon_b^{-1})}{m_d/\epsilon_b}}+\frac{2\ ln(2m_d\cdot n\cdot \delta^{-1}\cdot \epsilon_b^{-1})}{3\cdot m_d/\epsilon_b}.
$$
Therefore, since the maxima of the quantile $q(1-q)$ is at $q=1/2$, this is a boundary of the quantile interval $[1/2,1]$, so we could know that for any quantile fall in two adjacent queried quantiles, its first term should be bounded by one of the two adjacent quantiles. Then we have for all the quantiles in the interval $[t_l,t_r]$:
$$
\left\vert q^{E_i}(v) -q^{D_i}(v)\right\vert \le \sqrt{\frac{2q^D(1-q^D)\ln(2m_d\cdot n\cdot \delta^{-1}\cdot \epsilon_b^{-1})}{m_d/\epsilon_b}}+\frac{2\ ln(2m_d\cdot n\cdot \delta^{-1}\cdot \epsilon_b^{-1})}{3\cdot m_d/\epsilon_b} + (t_r-t_l)/m_d,
$$
Notice that $\ln(ax)/x$ is monotonically decreasing when $ax>e$, since we have $m_d/(t_r-t_l)>e$, we get the following relations:
\begin{align*}
    \left\vert q^{E_i}(v) -q^{D_i}(v)\right\vert &\le \sqrt{\frac{2q^D(1-q^D)\ln(2m_d\cdot n\cdot \delta^{-1}\cdot \epsilon_b^{-1})}{m_d/\epsilon_b}}+\frac{2\ ln(2m_d\cdot n\cdot \delta^{-1}\cdot \epsilon_b^{-1})}{3\cdot m_d/\epsilon_b} + (t_r-t_l)/m_d \\
    & \le \sqrt{\frac{2q^D(1-q^D)\ln(2m_d\cdot n\cdot \delta^{-1}\cdot (t_r-t_l)^{-1})}{m_d/(t_r-t_l)}}+\frac{2\ ln(2m_d\cdot n\cdot \delta^{-1}\cdot (t_r-t_l)^{-1})}{3\cdot m_d/(t_r-t_l)}\\
    & \quad\quad\quad + (t_r-t_l)/m_d\\
    & \le \sqrt{\frac{2q^D(1-q^D)\ln(2m_d\cdot n\cdot \delta^{-1}\cdot (t_r-t_l)^{-1})}{m_d/(t_r-t_l)}} +
    \frac{2\ ln(2m_d\cdot n\cdot \delta^{-1}\cdot (t_r-t_l)^{-1})}{3\cdot m_d/(t_r-t_l)} \\&\quad \quad \quad 
    +\frac{ln(2m_d\cdot n\cdot \delta^{-1}\cdot (t_r-t_l)^{-1})}{3\cdot m_d/(t_r-t_l)}\\
    &\le \sqrt{\frac{2q^D(1-q^D)\ln(2m_d\cdot n\cdot \delta^{-1}\cdot (t_r-t_l)^{-1})}{m_d/(t_r-t_l)}}+
    \frac{ln(2m_d\cdot n\cdot \delta^{-1}\cdot (t_r-t_l)^{-1})}{ m_d/(t_r-t_l)}.
\end{align*}
Since the values we query are taken from the data company and are all multiples of $\epsilon_b /m_d$ (the distance between two adjacent points in our queries is always $\epsilon_b/m_d$ times a power of 2). Therefore all the quantile points we query all satisfy the above inequality. If we shade the quantiles with function $s_{m_d/(t_r-t_l),n,\delta}$.
\end{proof}
\end{comment}
